Learning Temporal Dynamics from Cycles in Narrated Video

Learning to model how the world changes as time elapses has proven a challenging problem for the computer vision community. We propose a self-supervised solution to this problem using temporal cycle consistency jointly in vision and language, training on narrated video. Our model learns modality-agnostic functions to predict forward and backward in time, which must undo each other when composed. This constraint leads to the discovery of high-level transitions between moments in time, since such transitions are easily inverted and shared across modalities. We justify the design of our model with an ablation study on different configurations of the cycle consistency problem. We then show qualitatively and quantitatively that our approach yields a meaningful, high-level model of the future and past. We apply the learned dynamics model without further training to various tasks, such as predicting future action and temporally ordering sets of images. Project page: https://dave.ml/mmcc

==> text/intro.tex <==

%%%%%%%%% BODY TEXT
\section{Introduction}

% \setlength{\epigraphwidth}{\columnwidth}
% \epigraph{Making predictions is very difficult,\\especially about the future.}{\textit{Niels Bohr}}

% - motivation (example, connection to humans)
% - what we do
% - how we do it
% - how we evaluate it / our contributions

% refer to the teaser, talk about how predicting the future is important and hard
% and text might help reduce the ambiguity, would be good to point that out at the beginning
% then say directly that using information in vision and text, we propose cycles to discover the good future transitions
% then paragraph 3 and on are the same

% \cs{add one sentence before referring to Figure 1, what about: Prediction the future is an important problem in computer vision and has recently received a lot of attention + add a couple of references}

Predicting the future is a central problem in computer vision \cite{ebert2017self,finn2017deep,jayaraman2015learning,lee2018stochastic,mathieu2015deep,vondrick2016generating}.
%cs: I remove this argument, it is not super convincing 
%and I don't think it adds to the paper.
%, perhaps since predictive abilities have been proposed as a fundamental mechanism in our brains that drives how we represent the world internally, how we reason about it, and how we act upon it \cite{predictioncognitionandthebrain, huang2011predictive}. 
However, previous methods have largely focused on predicting fixed, small offsets into the future. To understand why this formulation is flawed, consider Figure~\ref{fig:teaser}. This figure shows a frame \textbf{(a)} from a video at time $t$ and three frames at times $>t$. Which one of these should be the output of a model that predicts the future? Option \textbf{(d)} is closest to the future that humans are likely to imagine by thinking about high-level transitions in time. However, with few exceptions~\cite{tap}, previous work focuses on predicting frames such as option \textbf{(b)}, which occur in the immediate future. This design choice limits the types of temporal transitions that can be learned by models and hurts performance, since adjacent frames are liable to be noisy or uninteresting.

% The ability to predict temporal dynamics  \jw{If we'd like to have a sentence like this, we may want to put it at the beginning of the intro.  The ability to ***. But to set it up right is non trivial. Figure 1 shows ***. Previously methods apparently didn't do it right and it has hurt them in terms of ***.} 

% \jw{Here we should probably mention that temporal consistency is important and useful. It has also been studied in multiple recent works. But we do it with text. This is key. very important. as shown in Figure 1 too. Text really helps to disambiguate the challenging problem.} 

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/teaser_onerow_text.png}
\vspace{0.2em}
\caption{\textbf{Predicting the future is challenging.} Given a frame \textbf{(a)} at time $t$, previous work focuses on predicting future frames at a fixed offset, such as \textbf{(b)}. However, these frames are often either redundant or stochastic, motivating the prediction of subsequent {\em informative} frames. Choosing such a frame is highly non-trivial. Aided by the textual information in narrated video, we can distinguish between visually distinct, but irrelevant, future frames such as \textbf{(c)} and pertinent ones \textbf{(d)}. We propose learning these dynamics by solving a temporal cycle consistency problem.}
\label{fig:teaser}
\vspace{-1.5em}
\end{figure}

To address these shortcomings and train a better predictive model, we introduce a multi-modal self-supervised cycle consistency task. Cycle consistency has been exploited as a learning signal freely available in video for solving problems such as object tracking~\cite{jabri2020space,wang2019learning}, action recognition~\cite{dwibedi2019temporal}, and even synthesis~\cite{Recycle-GAN}. In contrast to previous work, our formulation operates on minutes of video instead of seconds, and leverages information in multiple modalities to make more abstract, higher-level predictions in latent space. Rather than being trained to predict the future at fixed offsets, our model chooses how far into the future (and past) to predict in order to satisfy its objective.

% To address these shortcomings and imbue machines with stronger predictive abilities, we introduce a self-supervised temporal cycle consistency task, which requires a model to learn latent predictive models of the future and past which undo each other. Recent work has examined temporal cycles as a natural learning signal freely available in video for solving problems such as short-term object tracking~\cite{jabri2020space,wang2019learning}, action recognition~\cite{dwibedi2019temporal}, and even future frame synthesis~\cite{Recycle-GAN}. Importantly, we propose to incorporate textual information into temporal cycles, allowing our model to learn high-level and semantic concepts from real world video data. After training, our model can be used as-is to solve various tasks which rely on future prediction. \de{rework this paragraph to read more clearly as - we would like to train a machine to predict the future in a way that better aligns with how humans might do so. cycles have been used before to learn about low-level, very short term dynamics (flow, tracking). we propose a cycle formulation that uses info in viz+text to learn a model which makes high-level predictions about the future in a learned latent space}
% \chen{``abstract'' is a bit vague, should we use ``high-level'' as in abstract?} 

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{figs/attn_alt.png}
% \caption{\textbf{Cycles as repeated applications of soft attention:} We cast the problem of finding cycles in narrated video as end-to-end differentiable, repeated applications of soft attention. First, we embed all \colorbox{lpink!50}{visual} and \colorbox{lblue!50}{textual} nodes with networks $\Phi_V$ and $\Phi_T$. We compute attention between the start node's representation and all nodes in the other modality (here, text) to give a \colorbox{yellow!30}{cross-modal correspondence}. Information from both modalities is concatenated and passed into an MLP $g_\text{fwd} \circ f$. This outputs a latent prediction of \colorbox{green!30}{the future}, which uses attention to compute a visual future as a weighted combination of all possible nodes. The process is then repeated to go \colorbox{green!30}{backward in time}, replacing $g_\text{fwd}$ with $g_\text{back}$. The loss $\mathcal{L}_\text{cycle}$ trains the model's final output to close the cycle by predicting the start node. \de{modify as discussed on call: left side shows cycle graphically, right side blows up one temproal edge which is the same in both directions}}
% \label{fig:breakdown} 
% \end{figure*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{figs/new_approach.png}
% \vspace{0.1em}
% \caption{\textbf{Cycles as repeated applications of soft attention:} On the left, \textbf{(a)} shows our cycle formulation, starting from a moment in video. Note that text and video are frequently misaligned, as depicted. On the right, \textbf{(b)} shows the architecture of a temporal edge in detail. We embed all \colorbox{lpink!50}{visual} and \colorbox{lblue!50}{textual} nodes with $\Phi_V$ and $\Phi_T$. We then compute the \colorbox{yellow!30}{cross-modal node} corresponding to the start node with attention across the other modality. Both node representations are passed into an MLP $g_\text{fwd} \circ f$, which predicts \colorbox{green!30}{the future} using attention across the start modality. The process is then repeated to go \colorbox{green!30}{backward in time}, replacing $g_\text{fwd}$ with $g_\text{back}$. Our loss $\mathcal{L}_\text{cycle}$ trains the model's final output to close the cycle by predicting the start node.}
% \label{fig:breakdown} 
% \end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/fig2_b_only_midarrows_cordelia.png}
\vspace{0.1em}
\caption{%
{%
\setlength{\fboxrule}{1pt}%
\setlength{\fboxsep}{2pt}%
{%
\setlength{\fboxrule}{0.5pt}%
\setlength{\fboxsep}{1.5pt}%
\textbf{Learning temporal dynamics with cycles:} Given the \colorbox{lpink!50}{image} second from left as a \fcolorbox{darkpink}{white}{starting node},} our model finds corresponding \colorbox{lblue!50}{text}, \emph{``add soy sauce to the chicken''}, to build a \fcolorbox{lgreen}{white}{start state}. From this, our model predicts a future image and again builds a multi-modal state. Finally, our model predicts a past image from the future state. The discrepancy between this prediction of the past and the start image gives our \textcolor{davered}{\textbf{cycle-consistency loss}}. This final prediction is the result of a composition of multiple \textcolor{green}{\textbf{temporal}} and \textcolor{yellow}{\textbf{cross-modal}} edges, so our model can be trained end-to-end. Note that we use soft attention in practice to compute edges so that the process is differentiable.}}
\label{fig:tempdyn} 
\vspace{-1.5em}
\end{figure} %
Concretely, our model accepts as input a start state in the form of a frame from a video or a text utterance. It uses an attention mechanism to find a correspondence in the other modality, then uses information from both modalities to predict a future state in latent space, also with attention. From this future state, the model predicts a past state in a similar manner. We train our model such that these future and past predictions, when composed, lead back to the original start state. The only temporal loss used to train our model is the negative log-likelihood assigned to cycling back to the start state. We depict this cycle in Figure \ref{fig:tempdyn}. % \de{make this read more smoothly}
% \cs{say on whar precisely the cross-entropy is computed}

In Figure~\ref{fig:teaser}, only \textbf{(d)} is a viable solution to our cycle formulation. Selecting \textbf{(c)} as a future would not allow the model to return to \textbf{(a)}, since the two frames are unrelated. On the other hand, because the model does not know which modality its input comes from --- and therefore must operate equally on vision and language --- it is discouraged from selecting lower-level future frames such as \textbf{(b)}, which likely do not accompany a predictable change in text. Our hypothesis, which our experiments support, is that models which make high-level, significant predictions of the future and past will emerge as a solution to the cycle problem, as such predictions are easily inverted in either modality. %\de{make last sentence more concrete} %  (we can predict likely pasts as well as likely futures)

Our main contribution is the multi-modal temporal cycle consistency formulation and the improved predictive models learned by solving it. To evaluate our model, we:
\begin{itemize}
    \item Demonstrate that our model's predictions capture meaningful transitions between frames in video, visualizing discovered cycles and ranking transitions by their estimated likelihood. 
    \item Quantitatively show that our model's predictions are more temporally salient than previous work by training a temporal classifier on pairs of present and predicted future frames. \de{how is this, chen?} \item Apply our model without fine-tuning to downstream tasks such as future action anticipation and temporal ordering of sets of images, and justify our formulation with an extensive ablation study. 
\end{itemize}% \de{phrase less abstractly} \chen{there is a gap between our model being more temporal salient (subjective, no quantitative eval), to improved practical performance (such as future action classification). We might want to explain this is due to our model automatically discovers ``better'' ground truth of future and past, and that our model is able to do so over a longer time span.}
% Our model is trained on a large collection of unconstrained real-world data, and outperforms previous self-supervised approaches to prediction on all considered tasks. In the remainder of this paper, we describe the cycle consistency formulation and its evaluation in detail. 

Since our model is better able to capture complex long-term temporal dynamics, we outperform previous state-of-the-art on all tasks we consider. \de{not sure if bullet points are good here? maybe too long?}

% \jw{I'd add a few sentences to discuss the datasets and results.} \cs{agreed with jw}

% Prediction has been proposed as a fundamental mechanism in our brains that drives how we represent the world internally, how we think about it, and how we act upon it \cite{predictioncognitionandthebrain}. For example, consider the case of a baking sheet with cookies just pulled out of the oven. We represent the cookies as ``too hot'' since we predict they would burn our tongue and fingers if we tried to eat them right away. We instead choose to wait until they cool down, predicting that this experience would be more enjoyable. Some cognitive scientists even propose a framework \cite{huang2011predictive} where errors in predictions form the basis of our cognition: a young child who has never made the mistake of eating a too-hot cookie is more likely to do so. 

% Training a machine to model the temporal dynamics of our world has proven a challenging task. Previous approaches focus on generating future frames of video given a history \cite{vondrick2016generating}, anticipating future actions \cite{vondrick2016anticipating, oops}, and taking into account the uncertainty of possible near futures \cite{tap}. However, naively learning to predict pixels or representations some fixed offset into the future fails to produce strong results, especially in complex real-world data, since the future is too often unpredictable or uncertain. When we predict the future, we ignore irrelevant noise and focus on semantic transitions between states ({\em e.g.} scooping cookie dough $\to$ putting tray in oven). In this paper, we train a self-supervised machine to learn a semantic model of temporal dynamics and use this model to predict the future.

% Our approach uses temporal cycle consistency as a cue to discover semantic transitions between states in video. Our model takes in as input a start state in the form of a frame from a video and learns to select a future state, using both visual and textual (cross-modal) information. From this future state, the model predicts a past state in a similar manner. We train our model such that these forward and backward predictions, when composed, lead back to the original start state. We show that a model of semantic temporal dynamics emerges as a solution to this problem, since this type of transition is easily inverted (we can predict likely pasts as well as likely futures). \de{Discuss role played by text info}

% To demonstrate that a model trained with this self-supervised constraint discovers temporal dynamics, we use our learned model to detect temporally salient (predictable) moments in video, order shuffled sets of video clips, predict actions that caused a transition between two states, retrieve futures conditioned on user input, and plausibly interpolate between far-apart moments in video. In the remainder of this paper, we describe the cycle consistency formulation and its evaluation in detail. \de{contributions? clearer distinction from prior work? be clearer about what we want to learn}


% \cs{high-level comment introduction: I agree with JW's comments; figure 1 is very nice and clearly illustrates the approach; could we have a figure 2 on page 2 which we refer to in the introduction which gives us a good idea of the approach; I feel that the description in the intro is a little vague}

% \cs{current figure 2: it is hard to read; the within modality cycles are not entirely clear from the figure 2, maybe we could show in figure 2 only (c) and maybe it clearer including the loss }

% \cs{figure 3 is very hard to read/understand; would there be a way to improve it?}


% \de{skeleton, contributions and experiments}





